Torsion Resistant Strain Limiting Layers Enable High Grip Strength of Electrically-Driven Handed Shearing Auxetic Grippers

Soft grippers have demonstrated a strong ability to successfully pick and manipulate many objects. A key limitation to their wider adoption is their inability to grasp larger payloads due to objects slipping out of grasps. We have overcome this limitation by introducing a torsionally rigid strain limiting layer (TR-SLL). This reduces out-of-plane bending while maintaining the gripper's softness and in-plane flexibility. We characterize the design space of the strain limiting layer and Handed Shearing Auxetic (HSA) actuators for a soft gripper using simulation and experiment. The inclusion of the TR-SLL with HSAs enables HSA grippers to be made with a single digit. We found that the use of our TR-SLL HSA gripper enabled pinch grasping of payloads over 1 kg. We demonstrate a lifting capacity of 5 kg when loading using the TR-SLL. We also demonstrate a peak pinch grasp force of 5.8 N, and a peak planar caging force of 14.5 N. Finally, we test the TR-SLL gripper on a suite of 43 YCB objects. We show success on 37 objects demonstrating significant capabilities.

==> intro-back.tex <==
\section{Introduction}
A key component of human’s remarkable grip is that our fingers can simultaneously bend while being resistant to torsion and lateral loading. Soft robotic fingers have focused on emulating the ability of human and other biotas compliance when bending and found great success in the academy and industry as a result\cite{rus2015design}. This bending motion defines a plane of desired movement for the finger or actuator. While in plane bending and compliance are desired, movement normal to this plane, or out-of-plane deformation has been identified as a major limiter in soft robotic systems. 
Soft grippers ability to grasp and manipulate heavy objects is limited by out-of-plane deformations. With caging or parallel-to-gravity lifts, soft robotic systems have been able to lift car tires and dumbbells\cite{li2017fluid,li2019vacuum,li2022scaling}. 
 When perpendicular to the gravity field, or when large moments are present, soft grippers ultimately lose their grasp from deformations and twists. The out-of-plane finger deformations introduce uncertainty in the position of the grasped object. Localization relative to the arm can also be challenging when successfully grasping heavy loads because of deformations in the gripper. This work shows how a torsion resistant strain limiting layer (TR-SLL) integrated into an electrically-driven handed shearing auxetic gripper can exceed payloads of 1 kg when grasping using the fingers as demonstrated in Fig. \ref{fig:hero}(a), and increase the lifting capacity to 5 kg when loading through the continuous skeleton as shown in Fig. \ref{fig:hero}(b).

%hero figure
\begin{figure}[t]
    \centering
    %\hfill
    \includegraphics[width=1\linewidth]{media/Herofig.png}
    %\captionsetup{justification=centering}
    \caption{We create a new Torsion Resistant Strain Limiting Layer (TR-SLL) that can be added to an existing soft gripper. It increases the gripper's resistance to torsion, allowing the gripper to lift larger payloads. Additionally, we can load the skeleton of the TR-SLL directly, dramatically increasing lifting capacity. Here we create a Handed Shearing Auxetic (HSA)-based gripper using the TR-SLL and two quasi direct drive motors. in a) We show the HSA-based TR-SLL gripper lifting a 1 kg mass using a planar caging grasp. In b) we lift a 5 kg dumbbell using the skeleton from the TR-SLL, the maximum payload capacity of the UR5 robot arm.}
    \label{fig:hero}
    %\vspace{-0.5cm}
\end{figure} 

The most common place in soft robotics where strain limiting layers appear is in Pneu-nets\cite{mosadegh2014pneumatic}. The standard Pneunet uses a simple rectangular beam as the strain limiting layer (SLL). Rectangular cross sections have low second moments of inertia in one direction, allowing them to bend in the thin direction. While in theory, this would make them able to resist deformations along their thick direction, in practice, these structures have a low resistance to torsion. This causes any out-of-plane loading to generate a twist in the SLL and gripper.

For electrically-driven handed shearing auxetic grippers, a torque must be resisted to generate extension or bending of the HSA. A strain limiting layer has typically been ommited in favor of a second, opposite handed HSA \cite{chin2018compliant,chin2019simple}. In another work, rigid cable elements in addition to a second HSA are used to stiffen the system to undesired bending modes\cite{chin2020multiplexed}. The second HSA increases the moment of inertia, reducing non-planar bending modes. However, this does not reduce out-of-plane deformations as much as the TR-SLL work presented here. These works also demonstrate lower payload capacities when looking at solely HSA-based gripping. Additionally, these systems need a non-rotating grasping surface to be added to the gripper whereas the TR-SLL in this work serves both purposes.

Several strategies have emerged for improving the out-of-plane performance of soft grippers through the SLL. One approach focuses on changing the material distribution by using multi-material topology optimization\cite{wang2022topology}. Another approach discritizes the SLL and inserts hinges to allow a thicker material to still bend \cite{lotfiani2020torsional}. The first still experiences large out-of-plane deformations while demonstrating smaller increases in torsional stiffness. The second uses hinge-based strain limiting layers (SLL) which can reduce the structures ability to conform to objects compared to the continous design presented here.

We focus on using advancements from the field of compliant mechanisms to change the geometry of the SLL. We use triangulated beams as the torsion resistant strain limiting layer (TR-SLL) of Pneu-net. These triangulated beams resist torsion but allow bending on planar and spherical surfaces \cite{rommers2021new,naves2017building}. While one might expect the triangles along the beam to localize the deformation to interfaces between triangles, the structures deform over their entire length, with all sides of the triangle deforming when bent. Rhombus and honeycomb cross-sections have been integrated into robots using pneumatic air bladders \cite{Jiang2016Honeycomb,Jiang2021Hierarchical} and tendons \cite{childs2021rhombus} however both systems demonstrate smaller payloads than this work. The triangularized beams act as a continuum structure with enhanced stiffness to out-of-plane bending and torsion. This behaviour has a close analog with the human hand in the tendons and bones, however this work produces a continuous skeleton instead of discretized elements.

We integrate the TR-SLLs into electrically-driven handed shearing auxetic grippers and provide a step-by-step guide for integrating the TR-SLLs. Next, we perform a parametric sweep on the TR-SLLs to provide a design guide. We found that triangles close to equilateral best resisted torsion. We found in plane stress concentrations decreased with triangle count while stress from torsion followed that trend above 10 triangles per 100mm span. We tested the integrated gripper on a cylindrical pull test and found that the addition of the TR-SLL enabled grip forces above 5N for pinch grasps and above 14N for caging grasps. Finally, we tested the gripper by picking up a weighted structure entirely using the sides of the gripper. As seen in Fig. \ref{fig:hero}, the TR-SLL gripper can pick up a 5 kg weight (the max capacity of the UR5) using lateral loading. 


In this paper we:
\begin{itemize}
    \item Model key parameters to understand a torsion resistant strain limiting layer
    \item Analyze the design space of handed shearing auxetics through mechanical characterization
    \item Integrate the TR-SLL with handed shearing auxetics to build a soft gripper and demonstrate its enhanced payload capacity
\end{itemize}

\section{Background}
Soft robotics researchers have attempted to improve the out-of-plane performance of soft grippers using several techniques. 
One method is to redesign the gripper as a whole. This can involve  putting a skeleton around the entire gripper\cite{scharff2019reducing}. However, this requires significantly more input energy to reach the same normal force output and demonstrates smaller lifting capacity. Another method involves optimizing the design of individual cells to improve torsion resistance\cite{su2022optimizing}.

Active strain limiting layers are another area of research. Many of these change their SLL stiffness through phase change \cite{zhang2019fast}, jamming chain, \cite{jiang2019chain} or through the thermoelectric properties of Field's metal \cite{buckner2019enhanced,gunawardane2022thermoelastic} or by heating hydrogels, causing them to swell\cite{visentin2021selective}. Additionally, work has been done to use jamming to increase a gripper's ability to grasp objects and increase out-of-plane grip strength\cite{crowley20223d}. 






Our solution allows a simple passive SLL made from a single material to be easily integrated into existing soft gripper designs. It demonstrates a large torsional spring constant and high in-plane compliance. It can be made with a low cost 3D printer and can be integrated into a variety of different soft gripper designs.


\section{Derivation of the effect of Torsion on Antipodal Gripping for Soft Bodies}

In this section we characterize the three common failure modes for soft grippers. We introduce the idea that deformations from moments are often a dominant term, and then map equations to describe this failure mode.

%Soft Failure Modes
\begin{figure}
    \centering
    %\hfill
    \includegraphics[width=1\linewidth]{media/GripperFailureModes.png}
    %\captionsetup{justification=centering}
    \caption{We demonstrate the common failure modes for soft robotic grasping. On the right we can see a simplified gripper grabbing a cylinder using an antipodal grasp. Only the Strain Limiting Layer and soft gripping material between the SLL and object is shown (not to scale). On the left, three common failure modes are shown; slipping due to low normal forces, twisting due to torsional deformation in the SLL, and shearing of the soft material. The maximum payload capacity for a this gripper is governed by the minimum of the set of these conditions. By understanding these limits, we can better inform gripper design. By including the TR-SLL, we dramatically increase our soft grippers resistance to twist. This allows it to lift larger payloads while having a better understanding of where the object is in our grasp.}
    \label{fig:failureModes}
    %\vspace{-0.6cm}
\end{figure}

Antipodal gripping is a widespread application for soft robotic grippers. It involves picking up an object through two opposite points. There are three common limits to a soft grippers ability to perform an antipodal grasp; insufficient normal force, slippage due to torsional deformation, and shearing of the soft layer. All three of these modes as well as an example antipodal grasp can be seen in Fig. \ref{fig:failureModes}. The minimum of these three modes govern the payload capacity for an antipodally lifted object. If the payload minimum is governed by insufficent normal force, the force a gripper can lift is shown in Eq. \ref{eq:staticForce}.

\begin{equation}
     F_{static} = \mu F_n
     \label{eq:staticForce}
\end{equation}

where $F_{static}$ is the maximum force a gripper can lift, $\mu$ is the coefficient of static friction, and $F_n$ is the normal force the gripper applies as shown in Fig. \ref{fig:failureModes}. If instead the gripper is just at the limit of slip from twisting, we get:

\begin{equation}
     M = {F_gr}
     \label{eq:staticTorque}
     %\vspace{-0.15cm}
\end{equation}

\begin{equation}
     M = \kappa\theta
     \label{eq:Torque}
     %\vspace{-0.15cm}
\end{equation}


where $M$ is the moment on the SLL, $F_g$ is the gravitational force from the object, $r$ is the distance from the neutral axis of the gripper to the object, $\kappa$ is the torsional spring constant from twisting failure, and $\theta$ is the angle of twist relative to the normal force. These can be seen labeled in the twisting failure modes in Fig. \ref{fig:failureModes}. If we assume there is some small vertical deformation $x$ as the gripper is loaded but no slip or rolling occur, we get Eq. \ref{eq:xsmallAng}.

\begin{equation}
     x = r\theta
     \label{eq:xsmallAng}
\end{equation}

Combining Eq. \ref{eq:staticTorque}, Eq. \ref{eq:Torque}, and Eq. \ref{eq:xsmallAng} we can solve for $F_g$ as a function of $x$:

\begin{equation}
    F_g = \dfrac{\kappa}{r_{t}^2} x 
    \label{eq:forceG}
\end{equation}

Where $\dfrac{\kappa}{r_{t}^2}$ is the effective stiffness of the TR-SLL. We can use the net torque requirement from the HSA to further enhance $F_g$. We intentionally choose a HSA chirality that resists objects slipping due to the gravity field, adding to the net force supported.

\begin{equation}
    F_g = \dfrac{\kappa}{r_{t}^2} x + \dfrac{c_{\tau}}{r_{h}}  \varphi
    \label{eq:forceG+HSA}
\end{equation}
where $c_{\tau}$ is the torsional spring constant as presented in \cite{good2021expanding}, $r_{h}$ is the distance from the center of the HSA to the grasping surface, and $\varphi$ which is the angle of twist of the HSA from the motor. As shown in Fig. \ref{fig:failureModes}, the HSA's contribution is represented with the opposite direction torque $M_{hsa}$ where the second half of Eq. \ref{eq:forceG+HSA} is equal to it.

\begin{equation}
    M_{hsa} =  \dfrac{c_{\tau}}{r_{h}}  \varphi
    \label{eq:torqueHSA}
\end{equation}

Shearing of the soft gripping material can be another concern and is defined when:
\begin{equation}
     \tau > \tau_{f} 
     \label{eq:shearStress}
     %\vspace{-0.15cm}
\end{equation}

where $\tau$ is the length of the shear vector in the material and $\tau_{f}$ is the shear fracture of the material. For this study delamination was seen for high mass objects.

Together, the minimum force value from Eq. \ref{eq:staticForce}, Eq. \ref{eq:forceG+HSA}, and Eq. \ref{eq:shearStress} govern the payload capacity of a soft gripper performing an anti-podal pick on a simple object. Since soft grippers often demonstrate out-of-plane deformation as a common failure mode, this work looks to Eq. \ref{eq:forceG+HSA} as a way to increase the payload capacity of soft grippers. This paper achieves this through the creation of a continuously-deformable torsion resistant strain limiting layer. 


